PEBBLE: Feedback-Efficient Interactive Reinforcement Learning via Relabeling Experience and Unsupervised Pre-training

Conveying complex objectives to reinforcement learning (RL) agents can often be difficult, involving meticulous design of reward functions that are sufficiently informative yet easy enough to provide. Human-in-the-loop RL methods allow practitioners to instead interactively teach agents through tailored feedback; however, such approaches have been challenging to scale since human feedback is very expensive. In this work, we aim to make this process more sample- and feedback-efficient. We present an off-policy, interactive RL algorithm that capitalizes on the strengths of both feedback and off-policy learning. Specifically, we learn a reward model by actively querying a teacher's preferences between two clips of behavior and use it to train an agent. To enable off-policy learning, we relabel all the agent's past experience when its reward model changes. We additionally show that pre-training our agents with unsupervised exploration substantially increases the mileage of its queries. We demonstrate that our approach is capable of learning tasks of higher complexity than previously considered by human-in-the-loop methods, including a variety of locomotion and robotic manipulation skills. We also show that our method is able to utilize real-time human feedback to effectively prevent reward exploitation and learn new behaviors that are difficult to specify with standard reward functions.

==> sections/intro_v1.tex <==

Deep reinforcement learning (RL) has emerged as a powerful method whereby agents are enabled to learn complex behaviors on their own through trial and error~\cite{quadrupedal,policy-search,robot-rl,alphago,in-hand-manip,qtopt,alphastar}. 
% \km{here, do you wanna refer some robotics applications only or other things like AlphaGo, AlphaStar, OpenAIFive?}\lms{we should probably refer to the things you mentioned, not only robotic applications :)}
Scaling RL to many applications, however, is yet precluded by a number of challenges. 
One such challenge lies in providing a suitable reward function.

For example, as sparse signals are often insufficient to train RL agents, real-world problems may require extensive instrumentation, such as
accelerometers to detect door opening~\cite{dagps}, thermal cameras to detect pouring~\cite{pouring}, or motion capture and object tracking~\cite{em-rl, progressive-nets, akkaya2019solving, peng2020learning}.
% {motion capture and object tracking~\cite{em-rl,progressive-nets}, accelerometers to detect door opening~\cite{dagps}, or thermal cameras to detect pouring~\cite{pouring}. 
% % \pa{these citations are all a bit old; it'd be nice to include more recent ones to get the point across that even today this is still true}
% } 

\replaced[id=LS]{Despite these costly measures, it may still be difficult to construct a suitable reward function. Reward exploitation is a prevalent concern in RL--algorithms often discover ways to achieve high returns with unintended, sometimes dangerous\lms{maybe add some citations here idk}, consequences. In general, there is nuance in how we might want agents to behave, such as obeying social norms, that are difficult to account for and communicate effectively through an engineered reward function~\citep{amodei2016concrete,implicit-preferences, reward-side-effects}. 
}{
However, even with these costly measures, it may still be difficult to construct a suitable reward function that elicits the desired behavior.
Consider training a household robot to cook a dish.
We must be concerned with \textit{how} the robot accomplishes the task, as reward exploitation may lead to unintended but dangerous consequences.
It is important, for example, that the robot does not break anything expensive, harm anyone, or set the kitchen aflame in the process. Generally, there is nuance in how we might want agents to behave, such as obeying social norms, that are difficult to account for and communicate effectively through an engineered reward function~\citep{amodei2016concrete,implicit-preferences, reward-side-effects}. \pa{maybe this can be shortened / simplified a bit, and be more focused on the message that reward mis-specification can have significant consequences, as has been studied blabla}}
%\km{sg but don't know the details of papers you mentioned;}
% Assume that we want to train a robot to make a food or drive cars via RL.  
% One can imagine that specifying the reward function for the agent to optimize becomes harder as the tasks we want the agent to achieve become more complex.
% Hence, it is important to consider how to specify the reward for complex tasks in a way that is not only precise about the task but also provides learning signal.

% \km{"learning signal" is a bit ambiguous. Feel like we need to consider both "what to achieve" (success) and "how" (in some desired way). And above example sounds like we can miss "how" if we only care about "what". So, my point is that specifying what would be easy but doing how is not. I like this paragraph but it would be nice to change the last sentence.. Let me think!}

% Instead of specifying a reward function, we train a reward model using human feedback as supervision. The agent then optimizes to maximize the predicted returns.\lms{one problem I have with this caption is that it could be used for any preference-based RL thing..maybe we need to add something that's particular to our method specifically}
%\km{better to merge paragarphs?}
%\lms{I think it's kinda nice as its own paragraph since it's a complete thought and and important point. I'm not quite sure if the last sentence here makes complete sense in the context, what do you think?}
% \km{Another thought; we can emphasize some case, where it is not trivial to design a reward even with full information about internal state of robot or agents? here is some example: 
% However, for some complex domains and tasks, 
% it is often difficult to construct a suitable reward function that leads to the desired behavior.
% For example, assume that we want to train agents for simple tasks (e.g. ``stand" or ``pick up a block"), and then move to more complex tasks (e.g. ``run" or ``stack the blocks").
% In this setting, 
% an additional challenge emerges: Specifying the reward function for the agent to optimize becomes harder as the tasks we want the agent to achieve become more complex.
% Naively one might consider providing a reward when the agent successfully performs the tasks, 
% but that could make learning very slow because agent cluelessly tries things until success was achieved (by luck).  
% Hence, it is important to consider how we will specify the reward for complex tasks in a way that is not only precise about the task but also provides learning signal.}\lms{+1 yep}
% \km{Basically, we can emphasize that hand-designed reward is not always informative to induce desired behavior.}
% In contrast, humans are able to learn sophisticated skills without such carefully engineered external supervision. 


We thus seek a general form of supervision that not only \textit{is sufficiently rich in learning signal} for the agent, but also \textit{precisely specifies the objective}.\replaced[id=LS]{When learning sophisticated skills, humans do not rely on hand-engineered reward functions, and yet these requisite properties are fulfilled.}{If we consider the forms of supervision available to humans in order to learn sophisticated skills, we do not rely on such carefully engineered reward functions yet these requisite properties are fulfilled.} \pa{throughout often sentences are a bit long / hard to follow, the sentence right before this comment is a good example --- it's a bit long, it's also confusing b/c in the previous sentenc we talked about supervision but then we write "such carefully engineered reward functions" which sounds as if it references the previous sentence, but it doesn't reall b/c there is no "reward" in the previous sentence...}
One way to give such supervision is to provide demonstrations, which the agent learns to follow via inverse reinforcement learning~\citep{ng2000irl,abbeel2004irl} or imitation learning~\citep{schaal1997learning,argall2009il}. However, suitable demonstrations are expensive, sometimes prohibitively so, to obtain ~\cite{collab-manip,online-movement-adaptation,traj-keyframe,vr-teleop}.
% However, this supervision can not be applicable to some cases, where it is hard to generate demonstrations.
% \lms{Maybe we should mention imitation learning here first, then talk about how giving binary feedback is way less difficult and interactive (so we can give a curriculum and correct for the agent's particular failures)} 
% \km{I added that part. what do you think?}

Instead of relying on explicit demonstrations, we often learn fairly autonomously, relying on occasional external feedback from a teacher who may guide progress through providing corrective or increasingly advanced instructions. 
Applying such a paradigm under the purview of training artificial agents has been studied in the context of human-in-the-loop RL~\cite{brodleyhitl,preference_drl,tamer,coach}, in which a human provides feedback to the agent's behavior and the agent uses this feedback to perform the task.
% \lms{add some short description?}. 
While these frameworks have been able to successfully utilize forms of interaction, 
human-in-the-loop RL has been challenging to scale because putting humans into the robot training loop is incredibly costly.
Popular approaches largely utilize on-policy RL algorithms due to their fundamental design~\cite{coach,deepcoach} 
or to mitigate the effects of a reward function that is learned online~\cite{preference_drl}. 
\lms{more citations}
\km{to mitigate ~ is a bit unclear b/c (1) COACH also considered non-stationarity issue (b) learning dynamics sounds like learning a transition dynamics.}\lms{better?} \ow{Still unclear I think.}
% The predominant challenge faced by these interactive approaches is that human feedback is costly, which is further exacerbated by the sample-efficiency of standard RL methods. 


% \lms{need to bring up issue of non-stationarity (maybe) another option is to just state that popular methods require using on-policy algorithms}
% \km{maybe, not here? one possible storyline is (1) we wanna develop efficient algorithm --> (2) we consider off-policy --> (3) but there is an issue of non-stationarity --> (4) talk about ideas to handle this issue?}


In this work, we aim to substantially reduce the amount of effort required for human-in-the-loop learning in order to guide agents in a manner that is easy, natural, and practical for humans. 
To this end, we present \metabbr: \textbf{R}elabeling \textbf{E}xperience with an \textbf{Ac}tive \textbf{T}eacher, a feedback-efficient RL algorithm by which learning is largely autonomous and supplemented by a handful of binary labels (i.e., preferences) provided by a human supervisor. Specifically, we do not assume the agent is privy to rewards from its environment. 
Instead, we learn a reward model on the data the agent collects by querying a teacher with two clips of behavior for which is preferable as proposed by ~\citet{preference_drl}.  \pa{preceding sentence hard to follow; also it's many times two clips not just two clips total, which might need more precise phrasing accordingly}
We then use a sample-efficient, off-policy RL method, Soft Actor-Critic (SAC; \citealt{sac}), to optimize a policy with respect to this reward model. To account for the non-stationarity in reward caused by learning the reward function online, we relabel all of the agent's past experience every time we update the model.
%{We then label all the agent's past experience with this model, constituting a replay buffer which we use to train a policy using a data-efficient, off-policy RL method, Soft Actor-Critic (SAC; \citealt{sac}). To account for the non-stationarity in reward caused by learning the reward function online, we reset and re-train our critic when significant shifts are detected. By using an off-policy method and leveraging the reward model to re-label experience, we reduce the amount of human involvement required.}
% \km{better to put this sentence at the above paragraph or remove?} 
To further reduce the role of the supervisor, we show that leveraging fully unsupervised pre-training, in which the agent relies only on intrinsic motivation to collect experience, greatly reduces the amount of human involvement by producing much more informative queries than those of undirected exploration.
% \km{just wanna make sure if you wanna remove the "In summary~"}
% In summary, our contributions are as follows: 
% \begin{itemize} [leftmargin=8mm]
% \setlength\itemsep{0.1em}
% \item An off-policy RL algorithm with relabeling for handling non-stationarity. 
% \item Feedback-efficient reward modeling via active learning. 
%  \item Unsupervised exploration to collect more informative experiences.
% \end{itemize}
% To further reduce the role of the supervisor, we introduce the following. First, we show that leveraging a fully unsupervised initial exploration phase, in which the agent relies only on intrinsic motivation to collect experience, greatly reduces the amount of human involvement by producing much more informative queries than those of undirected exploration. We also improve the active queries from the model by means of metric learning and careful sampling, which reduces the amount of feedback needed to learn our reward model.
% In summary, our contributions are as follows: 
% \begin{itemize} [leftmargin=8mm]
% \setlength\itemsep{0.1em}
% \item An off-policy RL algorithm with relabeling for handling non-stationarity. 
% \item Feedback-efficient reward modeling via active learning. 
%  \item Unsupervised exploration to collect more informative experiences.
% \end{itemize}
% % \ow{Is one of these three more significant than the others? From the intro it sounds like \#1 is the most novel contribution, in which case put it first.}

We evaluate \metabbr\, on a challenging suite of simulated robotic tasks involving long-horizon locomotion and manipulation skills. \metabbr\, outperforms ablations and prior methods in terms of both data and human efficiency by a substantial margin. \lms{hopefully we can make some claim about how we believe this brings us closer to deploying HILL algorithms in the real world or like something about being able to tackle more complex tasks than have been achieved before}


% \km{Under O1-O3, we will develop RL agents that can learn new skills building on behavioral priors for tasks, where we can specify rewards. 
% However, for some complex domains and tasks, 
% it is often difficult to construct a suitable reward function that leads to the desired behavior.
% For example, assume that we want to train agents for simple tasks (e.g. ``stand" or ``pick up a block"), and then move to more complex tasks (e.g. ``run" or ``stack the blocks").
% In this setting, 
% an additional challenge emerges: Specifying the reward function for the agent to optimize becomes harder as the tasks we want the agent to achieve become more complex.
% Naively one might consider providing a reward when the agent successfully performs the tasks, 
% but that could make learning very slow because agent cluelessly tries things until success was achieved (by luck).  
% Hence, it is important to consider how we will specify the reward for complex tasks in a way that is not only precise about the task but also provides learning signal.}
